Cosmological Halos: A Search for the Ionized Intergalactic Medium

Standard big bang nucleosynthesis predicts the average baryon density of the Universe to be a few percent of the critical density. Only about one tenth of the predicted baryons have been seen. A plausible respository for the missing baryons is in a diffuse ionized intergalactic medium (IGM). In an attempt to measure the IGM we searched for Thomson-scattered halos around strong high redshift radio sources. Observations of the radio source 1935-692 were made with the Australia Telescope Compact Array. We assumed a uniform IGM, and isotropic steady emission of 1935-692 for a duration between 10^7 - 10^8 years. A model of the expected halo visibility function was used in \chi^2 fits to place upper limits on \Omega_{IGM}. The upper limits varied depending on the methods used to characterize systematic errors in the data. The results are 2/sigma limits of \Omega_{IGM} < 0.65. While not yet at the sensitivity level to test primordial nucleosynthesis, improvements on the technique will probably allow this in future studies.

==> thesis_bib <==
@string{apj = "Astrophysical Journal"}
@string{apjl = "Astrophysical Journal Letters"}
@string{apjs = "Astrophysical Journal Supplement Series"}
@string{mnras = "Monthly Notices of the Royal Astronomical Society"}
@string{aap = "Astronomy and Astrophysics"}
@string{aaps = "Astronomy and Astrophysics Supplement Series"}
@string{aj = "Astronomical Journal"}
@string{nat = "Nature"}



@Article{sbbn91,
author ={T.P. Walker and G. Steigman and D.N. Schramm
and K.A. Olive and H. Kang},
journal = apj,
volume =376,
pages ={51},
year =1991
        }
@Article{cst95,
author ={C. Copi and D. Schramm and M. Turner},
journal = "Science",
volume =267,
pages ={192},
year =1995
        }
@Article{hel4,
author ={Y. Izotov and X. Thuan and V. Lipovetsky}, 
journal = apj,
volume =435,
pages ={647},
year =1994
        }
@Article{yang84,
author ={J. Yang and others },
journal = apj,
volume =186,
pages ={493},
year =1984
        }
@Article{spite84,
author ={F. Spite and M. Spite},
journal = aap,
volume =115,
pages ={56},
year =1984
        }
@Article{thorburn94,
author ={J. Thorburn}, 
journal = apj,
volume =421,
pages ={318},
year =1994
        }
@Article{song94,
author ={A. Songaila and others},
journal = nat,
volume =368,
pages ={137},
year =1994
        }
@Article{wamp96,
author ={E. Wampler and others},
journal = aap,
volume =316,
pages ={33},
year =1996
        }
@Article{webb97,
author ={J. Webb and others},
journal = nat,
volume =388,
pages ={250},
year =1997
        }
@Article{tytler96,
author ={D. Tytler and X. Fan and S. Burles},
journal = nat,
volume =381,
pages ={207},
year =1996
        }
@Article{burles96,
author ={S. Burles and D. Tytler},
journal = "Submitted to Science.",
year =1996
        }
@Article{hogan97,
author ={C. Hogan},
journal = "astro-ph/9712031",
        }

@Article{persic92,
author ={M. Persic and P. Salucci},
journal = mnras,
volume = 258,
pages ={14},
year =1992
        }
@Article{steidel87,
author ={C. Steidel and W. Sargent},
journal = apj,
volume = 318,
pages ={L11},
year =1987
        }
@Article{webb92,
author ={J. Webb},
journal = mnras,
volume = 255,
pages ={319},
year =1992
        }

@Article{giall92,
author ={E. Giallongo and S. Cristiani and D. Trevese},
journal = apj,
volume = 398,
pages ={L9},
year =1992
        }


 
% end of INTRO refs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@Article{sholo90,
author ={G. B. Sholomitskii and A. L. Yaskovitch},
journal ={Soviet Astronomy Letters},
volume =16,
pages ={383},
year =1990
        }
@Article{sholo91,
author ={G. B. Sholomitskii},
journal ={Soviet Astronomy},
volume =35,
pages ={15},
year =1991
        }
@Article{sholo92,
author ={G. B. Sholomitskii},
journal ={Soviet Astronomy},
volume =36,
pages ={222},
year =1992
        }
@Article{vallee90,
author ={J.P. Vallee},
journal =aap,
volume =239,
pages ={57},
year =1990
        }
@Article{turner91,
author ={E.L. Turner},
journal ={Astronomical Journal},
volume =101,
pages ={5},
year =1991
        }
@Article{odea91,
author ={C. P. O'Dea and S. A. Baum and C. Stanghellini},
journal ={The Astrophysical Journal},
volume =380,
pages ={66},
year =1991
        }
@Article{odea97,
author ={C. P. O'Dea},
journal ={Submitted to PASP.},
year =1997
        }
@Article{bbr84,
author ={M. Begelman and R. Blandford and M. Rees},
journal ={Rev. Mod. Phys.},
volume =56,
pages ={255},
year =1984
        }

@Article{gunn65,
author ={J.E. Gunn and B.A. Peterson},
journal ={The Astrophysical Journal},
volume =142,
pages ={1633},
year =1965
        }
@Article{peebles91,
author ={P.J.E. Peebles, D.N. Schramm, E.L. Turner, and R.G. Kron},
journal ={Nature},
volume =352,
pages ={769},
year =1991
        }
@Article{macho95,
author ={Alcock and others},
journal ={Physics Review Letters},
volume =74,
pages ={2867},
year =1995
        }
@Article{macho97,
author ={Alcock and others},
journal =apj,
volume =486,
pages ={697A},
year =1997
        }
@Article{shapiro94,
author ={Shapiro and others},
journal =\apj,
volume =427,
pages ={25},
year =1994
        }
@Article{haslam82,
author ={G. Haslam and others},
journal =aap,
volume =47,
year =1982
        }
@Article{ski85,
author ={R. Antonucci and J. Ulvestad},
journal =apj,
volume =294,
pages ={158A},
year =1985
        }

@Article{wiering93,
author ={M. Wieringa and others},
journal =aap,
volume =268,
year =1993
        }

@Article{katz96,
author ={N. Katz and others},
journal =apj,
volume =457,
pages ={L57},
year =1996
        }

@Article{SZ96,
author ={P. Andreani and others},
journal =apj,
volume =459,
pages ={L49},
year =1996
        }


@Article{david96,
author ={A. Davidson and G. Kriss and W. Zheng},
journal =nat,
volume =380,
pages ={47},
year =1996
        }


@Article{hog97,
author ={C. Hogan and S. Anderson and M. Rugers},
journal =aj,
volume =113,
pages ={1495},
year =1997
        }


@Article{jakob95,
author ={P. Jakobsen and others},
journal =nat,
volume =370,
pages ={35},
year =1995
        }

@Article{rem98,
author ={D. Reimers and others},
journal = "astro-ph/9707173",
        }

@Article{con90,
author ={J. Conway and T. Cornwell and P. Wilkinson},
journal =mnras,
volume =246,
pages ={490},
year =1990
        }

@Article{hog74,
author ={J. H\"ogbom},
journal =aaps,
volume =15,
pages ={417},
year =1974
        }

@Article{noord82,
author ={J. Noordam and A.G. de Bruyn},
journal =nat,
volume =84,
pages ={597},
year =1982
        }

@Article{pear84,
author ={T. Pearson and A. Readhead},
journal =aap,
volume =22,
pages ={97},
year =1984
        }

@Article{sault91,
author ={R.J. Sault and N.E.B. Killeen and M.J. Kesteven},
journal ="ATNF Technical Memo No. 39.3015",
year =1991
        }


@Article{sault94,
author ={R.J. Sault and M.H. Wieringa},
journal =aaps,
volume =108,
pages ={589},
year =1994
        }

@Article{sault95,
author ={R.J. Sault and P.J. Teuben and M.C. Wright},
journal ="ASP Conference Series",
volume =77,
pages ={433},
year =1995
        }

@Article{wier1992,
author ={M.H. Wieringa},
journal ="Experimental Astronomy",
volume =2,
pages ={203},
year =1992
        }

@Article{inhomo90,
author ={H. Kurki-Suonio and others},
journal =apj,
volume =353,
pages ={406},
year =1990
        }

@Article{scheuer95,
author ={P. Scheuer},
journal =mnras,
volume =277,
pages ={331},
year =1995
        }



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Todd refs below













 
uthor ={C.H. Nelson and Mark Whittle},
journal = apjs,
volume =99,
pages ={67},
year =1995
	}

@Article{schillizi,
author ={R.T. Schillizi and A.G. de Bruyn},
journal = nat,
volume =303,
pages ={26},
year =1984
    }

@Article{wardle,
author ={J.F.C. Wardle and R.L. Moore and J.R.P. Angel},
journal = apj,
volume =279,
pages ={93},
year =1984,
    }

@Article{rees,
author ={M.J. Rees},
journal = nat,
volume =211,
pages ={468},
year =1966
	}

@Article{bland,
author ={R.D. Blandford and A. K\"onigl},
journal = apj,
volume =232,
pages ={34},
year =1979
    }

@Article{cohen,
author ={M.H. Cohen and others},
journal = nat,
volume =268,
pages ={405},
year =1977
    }

@Article{pearson,
author ={T.J. Pearson and others},
journal = nat,
volume =290,
pages =365,
year =1981
    }

@Article{angel,
author ={J.R.P. Angel and others},
journal = apjl,
volume =206,
pages ={5},
year =1976
	}

@Article{anto93,
author ={R.R.J. Antonucci},
journal = {Ann. Rev. Astron. Astrophys.},
volume =31,
pages ={473},
year =1993
	}

@Article{urry,
author ={C.M. Urry and P. Padovani},
journal = {Proceedings of the Astronomical Society of the Pacific},
volume =107,
pages ={803},
year =1995
    }

@Article{anto84,
author ={R.R.J. Antonucci},
journal = apj,
volume =278,
pages ={499},
year =1984
	}

@Article{am85,
author ={R.R.J. Antonucci and J.S. Miller},
journal = apj,
volume =297,
pages=621,
year=1985
	}

@Article{ahm94,
author ={R.R.J. Antonucci and Todd Hurt and J.S. Miller},
journal = apj,
volume =430,
pages=210,
year=1994
    }


@Article{blietz93,
author ={M. Blietz and others},
journal = apj,
volume =421,
pages=92,
year=1994
    }

@Article{burstein86,
author ={D. Burstein and C. Heiles},
journal = apjs,
volume =54,
pages=33,
year=1986
    }

@Article{cag91,
author ={S. Caganoff and others},
journal = apjl,
volume =377,
pages=9,
year=1991
    }

@Article{cap1,
author ={A. Capetti and others},
journal = apj,
volume =446,
pages=155,
year=1995
    }

@Article{tz,
author ={C.N. Tadhunter and Z. Tsvetanov},
journal = nat,
volume =341,
pages ={422},
year =1989
    }

@Article{cap2,
author ={A. Capetti and others},
journal = apjl,
volume =452,
pages={L87},
year=1995
    }

@Article{card89,
author ={J.A. Cardelli and G.C. Clayton and J.S. Mathis},
journal = apj,
volume =345,
pages=245,
year=1989
    }

@Article{car89,
author ={C.L. Carilli and J.W. Drether and S. Conner and R.A. Perley},
journal = aj,
volume =98,
pages=513,
year=1989
    }

@Article{cimm93,
author ={A. Cimatti and others},
journal = mnras,
volume =264,
pages=421,
year=1993
    }

@Article{cimm95,
author ={A. Cimatti and S. di Serego Alighieri},
journal = mnras,
volume =273,
pages={L7},
year=1995
    }

@Article{aligh88,
author ={S. di Serego Alighieri and others},
journal = nat,
volume =334,
pages=593,
year=1988
    }

@Article{drape93,
author ={P.W. Draper and S.M. Scarrott and C.N. Tadhunter},
journal = mnras,
volume =262,
pages=1029,
year=1993
    }

@Article{clayton,
author ={G. Clayton and others},
journal = apjl,
volume =385,
pages=53,
year=1992
    }

@Article{code93,
author ={A. Code and others},
journal = apjl,
volume =403,
pages=63,
year=1993
    }

@Article{elvius78,
author ={A. Elvius},
journal = aap,
volume =65,
pages=233,
year=1978
    }

@Article{evans91,
author ={I. Evans and others},
journal = apjl,
volume =369,
pages=27,
year=1991
    }

@Article{francis91,
author ={P.J. Francis and others},
journal = apj,
volume =373,
pages=465,
year=1991
    }

@Article{gilmore,
author ={G. Gilmore and M.A. Shaw},
journal = nat,
volume =321,
pages=750,
year=1986
    }

@Article{giov88,
author ={G. Giovannini and L. Feretti and L. Gregorini and P. Parma},
journal ={Astronomy \& Astrophysics} ,
volume =199,
pages=73,
year=1988
    }


@Article{koski78,
author ={A. Koski},
journal = apj,
volume =223,
pages=56,
year=1978
    }

@Article{lynds91,
author ={R. Lynds and others},
journal = apjl,
volume =369,
pages=31,
year=1991
    }

@Article{mclean83,
author ={I.S. McLean and C. Aspin and S.R. Heathcote and M.J. McCaughrean},
journal = nat,
volume =304,
pages=609,
year=1983
    }

@Article{ma83,
author ={J.S. Miller and R.R.J. Antonucci},
journal = apjl,
volume =271,
pages=7,
year=1983
    }

@Article{mg90,
author ={J.S. Miller and R.W. Goodrich},
journal = apj,
volume =355,
pages=456,
year=1990
    }

@Article{gm89,
author ={R.W. Goodrich and J.S. Miller},
journal = apjl,
volume =346,
pages={L21},
year=1989
    }

@Article{mgm91,
author ={J.S. Miller and R.W. Goodrich and W.G. Matthews},
journal = apj,
volume =378,
pages=47,
year=1991
    }

@Article{pier94,
author ={E.A. Pier and R. Antonucci and T. Hurt and G. Kriss and J. Krolik},
journal = apj,
volume =428,
pages=124,
year=1994
    }

@Article{ahk,
author ={R.R.J. Antonucci and T. Hurt and A. Kinney},
journal = nat,
volume =371,
pages=313,
year=1994
    }

@Article{antoulv,
author ={R.R.J. Antonucci and J. Ulvestad},
journal = apj,
volume =294,
pages=158,
year=1985
    }

@Article{scarrott91,
author ={S.M. Scarrott and C.D. Rolph and R.W. Wolstencroft and C.N. Tadhunter},
journal = mnras,
volume =249,
pages=16,
year=1991
    }

@Manual{kinney,
author={Anne Kinney},
title={FOS Instrument Handbook},
organization={Space Telescope Science Institute},
edition={2.0},
year=1992
	}

@Manual{baum94,
author={S. Baum},
title={HST Data Handbook},
organization={Space Telescope Science Institute},
edition={1.0},
year=1994
    }

@Manual{paresce,
author={F. Paresce},
title={Faint Object Camera Instrument Handbook},
organization={Space Telescope Science Institute},
edition={3rd},
year=1992
       }

@Manual{nota,
author={A. Nota and others},
title={Faint Object Camera Instrument Handbook},
organization={Space Telescope Science Institute},
edition={7th},
year=1996
       }


@Article{baum88,
author={S. Baum and others},
journal=apjs,
volume=68,
pages=643,
year=1988
    }

@Article{pierce86,
author={M.J. Pierce and A. Stockton},
journal=apj,
volume=305,
pages=204,
year=1986
    }

@Article{shaw92,
author={M.A. Shaw and A.K. Tziuomis and A. Pedlar},
journal=mnras,
volume=256,
pages={p6},
year=1992
    }

@Article{stockton94,
author={A. Stockton and S.E. Ridgway and S.J. Lilly},
journal=aj,
volume=108,
pages=414,
year=1994
    }

@Article{tadhunter90,
author={C.N. Tadhunter and S.M. Scarrott and C.D. Rolph},
journal=mnras,
volume=246,
pages=163,
year=1990
    }


@Article{tadhunter92,
author={C.N. Tadhunter and others},
journal=mnras,
volume=256,
pages={p53},
year=1992
    }


@Manual{rosa,
author={M. Rosa},
title={FOS Instrument Science Report, CAL/FOS-114},
institution={STScI},
address={Baltimore, Md.},
year={1993}
	}

@Manual{hodge,
author={P.E. Hodge},
title={FOC Instrument Science Report, CAL/FOC-069},
institution={STScI},
address={Baltimore, Md.},
year={1994}
    }

@Article{pogge,
author={R. W. Pogge},
journal=apj,
volume=328,
pages=519,
year=1988
	}

@Article{snijders,
author={M.A.J. Snijders and H. Netzer and A. Boksenberg},
journal=mnras,
volume=222,
pages=549,
year=1986
	}

@Article{tmk92,
author={H.D. Tran and J.S. Miller and L.E. Kay},
journal=apj,
year=1992,
volume=397,
pages=452
	}

@Article{unger,
author={S.W. Unger and J.R. Lewis and A. Pedlar and D.J. Axon},
year=1992,
journal=mnras,
volume=258,
pages=371
	}

@Article{wnw,
author={B.J. Wills and H. Netzer and D. Wills},
journal=apj,
year=1985,
volume=288,
pages=94
	}

@Article{whittle88,
author={M. Whittle and others},
journal=apj,
year=1988,
volume=326,
pages=125
	}

@Article{derob90,
author={M.M DeRobertis and R.A. Shaw},
journal=apj,
year=1990,
volume=348,
pages=421
        }

@Article{evans93,
author={I. Evans and others},
journal=apj,
year=1993,
volume=417,
pages=82
        }

@Article{hmbb81,
author={T.M. Heckman and G.K. Miley and W.J.M van Breugel and H.R. Butcher},
journal=apj,
year=1981,
volume=247,
pages=403
        }

@Article{heck86,
author={T.M. Heckman and others},
journal=apj,
year=1986,
volume=311,
pages=526
        }

@Article{hutch88,
author={J.B. Hutchings and I. Johnson and R. Pyke},
journal=apjs,
year=1988,
volume=66,
pages=361
        }

@Article{inglis93,
author={M.D. Inglis and others},
journal=mnras,
year=1993,
volume=263,
pages=895
        }

@Article{jackson93,
author={N.J. Jackson and C.N. Tadhunter},
journal=aap,
year=1993,
volume=272,
pages=105
        }

@Article{dekoof,
author={S. de Koof and others},
journal=apjs,
year=1996,
volume=107,
pages=621
        }

@Article{barthel,
author={P. Barthel},
journal=apj,
year=1989,
volume=336,
pages=606
        }


@Article{tranetal95,
author={H.D. Tran and M.H. Cohen and R.W. Goodrich},
journal=aj,
year=1995,
volume=110,
pages=2597
        }

@Article{tran3,
author={H.D. Tran},
journal=apj,
year=1995,
volume=440,
pages=597
        }

@Article{vdb76,
author={S. van den Bergh},
journal=apjl,
year=1976,
volume=210,
pages={L63}
        }

@Article{young,
author={S. Young and others},
journal=mnras,
year=1996,
volume=279,
pages={L72}
        }

@Article{leahy91,
author={J.P. Leahy and R.A. Perley},
journal=aj,
year=1991,
volume=102,
pages=537
        }

@Article{leahy84,
author={J.P. Leahy and A.G. Williams},
journal=mnras,
year=1984,
volume=210,
pages=929
        }
@Article{morganti,
author={R. Morganti and N.E.B. Killeen and C.N. Tadhunter},
journal=mnras,
year=1993,
volume=263,
pages=1023
        }

@Article{murphy,
author={T.W. Murphy and others},
journal=aj,
year=1996,
volume=111,
pages=1025
        }

@Article{neff,
author={S.G. Neff and L. Roberts and J.B. Hutchings},
journal=apjs,
year=1995,
volume=99,
pages=349
        }

@Article{neugebauer,
author={G. Neugebauer and others},
journal=apjs,
year=1987,
volume=63,
pages=615
        }

@Article{ogle,
author={P.M. Ogle and others},
journal=apjl,
year=1997,
volume=482,
pages={L37}
        }

@Article{neff,
author={S.G. Neff and L. Roberts and J.B. Hutchings},
journal=apjs,
year=1995,
volume=99,
pages=349
        }

@Article{heck84,
author={T.M. Heckman and W.J.M van Breugel and G.K. Miley},
journal=apj,
year=1984,
volume=286,
pages=509
        }

@Article{machetto94,
author={F. Machetto and others},
journal=apjl,
year=1994,
volume=435,
pages=15
        }

@Article{nw95,
author={C.H. Nelson and M. Whittle},
journal=apjs,
year=1995,
volume=99,
pages=67
        }

@Article{pogge89,
author={R.W.Pogge},
journal=apj,
year=1989,
volume=345,
pages=730
        }

@Article{pogge93,
author={R.W. Pogge and M.M. DeRobertis},
journal=apj,
year=1993,
volume=404,
pages=563
        }

@Article{tandt89,
author={C. Tadhunter and Z. Tsvetanov},
journal=nat,
year=1989,
volume=341,
pages=422
        }

@Article{vrtilek,
author={J.M. Vrtilek and N.P. Carleton},
journal=apj,
year=1985,
volume=294,
pages=106
        }

@Article{whittle85,
author={M. Whittle},
journal=mnras,
year=1985,
volume=213,
pages=1
        }

@Book{osterbrock89,
author={D.E. Osterbrock},
title={Astrophysics of Gaseous Nebulae and Active Galactic Nuclei},
year=1989,
publisher={University Science Books},
address={Mill Valley, Ca.},
edition="2nd",
	}

@Book{saas,
author={R.D. Blandford and H. Netzer and L. Woltjer},
editor={T.J.-L. Courvoisier and M. Mayor},
title={Active Galactic Nuclei: Saas-Fee Advanced Course 20, Lecture Notes 1990},
year=1990,
publisher={Springer-Verlag},
    }


@Book{peter,
author={B.M. Peterson},
title={Active Galactic Nuclei},
publisher={Cambridge University Press},
year=1997,
}

@Book{robson,
author={I. Robson},
title={Active Galactic Nuclei},
publisher={Wiley \& Sons},
year=1996,
}

@Book{press92,
author={W.H. Press and S.A. Teukolsky and W.T. Vetterling and B.P. Flannery},
title={Numerical Recipes in FORTRAN},
year=1992,
publisher={Cambridge Univ. Press},
edition="2nd",
        }

@Inbook{wh85,
author={A.S. Wilson and T.M. Heckman},
year=1985,
publisher={University Science Books},
address={Mill Valley, Ca.},
title={Astrophysics of Active Galaxies and Quasi-stellar Objects}
	}

@Inbook{anto96,
author={R.R.J. Antonucci},
year=1996,
publisher={Cambridge University Press},
title={Cygnus A --- Study of a Radio Galaxy},
pages=56
}

@Inbook{hurt96,
author={T. Hurt},
year=1996,
publisher={Elsevier Science Ltd.},
title={Vistas in Astronomy: Proceedings of the Oxford Torus Workshop},
volume=40,
pages=149
}

